An Empirical Study for Vietnamese Constituency Parsing with Pre-training

In this work, we use a span-based approach for Vietnamese constituency parsing. Our method follows the self-attention encoder architecture and a chart decoder using a CKY-style inference algorithm. We present analyses of the experiment results of the comparison of our empirical method using pre-training models XLM-Roberta and PhoBERT on both Vietnamese datasets VietTreebank and NIIVTB1. The results show that our model with XLM-Roberta archived the significantly F1-score better than other pre-training models, VietTreebank at 81.19% and NIIVTB1 at 85.70%.

==> sections/1-introduction.tex <==
\section{Introduction}

==> sections/2-relatedwork.tex <==
\section{Related Work}


==> sections/3-method.tex <==
\section{Method}


==> sections/4-experiments.tex <==
\section{Experiments}

==> sections/5-analysis.tex <==
\section{Analysis}

==> sections/6-conclusion.tex <==
\section{Conclusion}
